ChartREG++: Towards Benchmarking and Improving Chart Referring Expression Grounding under Diverse referring clues and Multi-Target Referring

Referring expression grounding is a core problem in visual grounding and is widely used as a diagnostic of spatial grounding and reasoning in vision and language models, yet most prior work focuses on natural images. In contrast, existing chart referring expression grounding-related benchmarks remain limited: (1) they largely adopt bounding boxes, constraining localization precision for fine chart elements (2) they mostly assume a single and two referred target instances, failing to handle multi-instance target references; (3) the language expressions over-rely on textual cues or data-rank clues (4) they cover only a narrow range of chart types. To address these issues, we introduce a chart referring expression grounding benchmark that systematically supports multiple localization forms, multiple referred targets, diverse grounding cues and diverse chart types. Results across representative multimodal large models reveal a significant performance gap. We further introduce a code-driven synthesis pipeline that exploits the inherent alignment between plotting programs and rendered chart primitives to derive pixel accurate instance masks across chart element types and granularities. We train an instance segmentation model with the synthesized masks and integrate it into a general-purpose multimodal grounding framework. The resulting system consistently outperforms baselines on our benchmark and generalizes well to a ChartQA-derived real-chart grounding benchmark.

==> seg_grounding_ori.tex <==
\subsection{Segmentation Grounding}
\label{sec:seg_grounding_res}

In this section, we evaluate segmentation grounding on \textsc{ChartREG++}. 
Importantly, we separate methods by their supervision setting. 
The Sa2VA and SAM3-SoM baselines are evaluated in a zero-shot setting, while our two-stage pipeline uses a chart-specific candidate generator trained with masks synthesized by our method. 
Thus, the latter is not intended as a fair zero-shot comparison against general-purpose MLLMs; instead, it evaluates whether our synthesized masks can provide useful supervision for learning high-quality chart instance candidates.

\subsubsection{Models}
We evaluate two segmentation grounding paradigms. 
\textbf{E2E-based} methods use the Sa2VA~\cite{yuan2025sa2vamarryingsam2llava} family, which directly predicts dense masks from the input image and referring expression. 
Since these models do not output separated chart instances, we only report $\mathrm{mIoU}_{\text{union}}$ for them.

\textbf{Two-stage-based} methods decouple candidate generation and language alignment. 
The first stage generates instance mask candidates, and the second stage uses Set-of-Mark (SoM) prompting~\cite{yang2023setofmarkpromptingunleashesextraordinary} to let an MLLM select masks matching the referring expression. 
We include three candidate-generation settings. 
(1) \textbf{SAM3-SoM} uses the SAM3 segment-everything pipeline~\cite{carion2025sam3segmentconcepts} with ChartAgent-style post-processing, including area thresholding, mask-level NMS, removing composite masks, and filtering masks dominated by white background pixels. 
(2) \textbf{Ours-SoM (all segs)} uses a Mask2Former~\cite{cheng2022maskedattentionmasktransformeruniversal} model fine-tuned with masks synthesized by our primitive-tracing pipeline. 
The training data includes 40K randomly sampled ChartCoder~\cite{zhao-etal-2025-chartcoder} examples and the ECDBench~\cite{yang2025effectivetrainingdatasynthesis} training split. 
(3) \textbf{Ours-SoM (gold-category segs)} further keeps only candidates whose category matches the target category of the referring expression. 
This is an analysis setting that assumes access to the target category. 
We also report \textbf{Ours-SoM (Oracle)}, where predicted candidates are replaced by ground-truth masks of the target category, to estimate the upper bound of the SoM+MLLM alignment stage.

\subsubsection{Evaluation metrics}
For methods that output separated instance masks, we perform one-to-one matching between predicted and ground-truth masks using the Hungarian algorithm. 
For common element types, we use mask IoU as the similarity score and count a match as true positive if $\mathrm{IoU}\ge 0.5$. 
For thin-line elements, including Errorbar, BoxMedianLine, Line\_with\_Points, and Polar\_Line\_with\_Points, we use Boundary IoU averaged over $d\in\{1,2,4,8\}$.\footnote{The line-width distribution in our dataset mainly falls in the range of 1--15 pixels.}
We compute macro Precision, Recall, and F1 from TP/FP/FN. 
We also report $\mathrm{mIoU}_{\text{union}}$, the sample-wise IoU between the union of predicted masks and the union of ground-truth masks, which measures overall region coverage.

\subsubsection{Results}
As shown in Table~\ref{tab:seg_results}, zero-shot segmentation grounding remains difficult on \textsc{ChartREG++}. 
Both Sa2VA and SAM3-SoM obtain limited performance, showing that general-purpose segmentation grounding methods struggle with fine-grained chart elements and multi-target references.

Our synthetic-supervised \textbf{Ours-SoM (all segs)} achieves much higher scores than SAM3-SoM. 
This result should not be read as a fair zero-shot comparison, since our first-stage Mask2Former is trained with synthesized chart masks. 
Rather, it shows that our synthesis pipeline provides effective supervision for learning cleaner chart instance candidates, and that candidate quality is a key bottleneck in two-stage grounding. 
The gold-category setting further improves performance by reducing the candidate search space, while the oracle row still leaves a clear gap from perfect performance. 
This suggests that, beyond candidate generation, instance-level language alignment under diverse cues and multi-target expressions remains challenging.
